List Decodable Mean Estimation in Nearly Linear Time

Learning from data in the presence of outliers is a fundamental problem in statistics. Until recently, no computationally efficient algorithms were known to compute the mean of a high dimensional distribution under natural assumptions in the presence of even a small fraction of outliers. In this paper, we consider robust statistics in the presence of overwhelming outliers where the majority of the dataset is introduced adversarially. With only an $\alpha < 1/2$ fraction of "inliers" (clean data) the mean of a distribution is unidentifiable. However, in their influential work, [CSV17] introduces a polynomial time algorithm recovering the mean of distributions with bounded covariance by outputting a succinct list of $O(1/\alpha)$ candidate solutions, one of which is guaranteed to be close to the true distributional mean; a direct analog of 'List Decoding' in the theory of error correcting codes. In this work, we develop an algorithm for list decodable mean estimation in the same setting achieving up to constants the information theoretically optimal recovery, optimal sample complexity, and in nearly linear time up to polylogarithmic factors in dimension. Our conceptual innovation is to design a descent style algorithm on a nonconvex landscape, iteratively removing minima to generate a succinct list of solutions. Our runtime bottleneck is a saddle-point optimization for which we design custom primal dual solvers for generalized packing and covering SDP's under Ky-Fan norms, which may be of independent interest.

==> content/appbinary.tex <==
\subsection{Binary Decision Problem}

Upper bound on opt find primal feasible solution. 

Let $\Tr (A_{i^\ast} ) +\Tr (B_{i^\ast} ) := \min_i \Tr (A_i ) +\Tr (B_i )$  (I guess it is $A_{i^\ast}$ not $A_i^\ast$) and let 
\[
M= \frac 1 { \Tr (A_{i^\ast} ) +\Tr (B_{i^\ast} )} I_{\ell \times \ell} , \quad 
W = \frac 1 { \Tr (A_{i^\ast} ) +\Tr (B_{i^\ast} )} I_{m \times m}
\]
For $m > k$, we have $M, W$ primal feasible and 
\[
\Tr (M) +\Tr (W )  = \frac {\ell + m}  { \Tr (A_{i^\ast} ) +\Tr (B_{i^\ast} )} .
\]
\bigskip 

Lower bound on opt, find dual feasible solution. 
\[
w_i = 
\begin{cases} 
\frac {1}  { \Tr (A_{i^\ast} ) +\Tr (B_{i^\ast} )}  & \text{ if } i= i^\ast \\
0& \text{ otherwise} 
\end{cases}
\]
Then 
\[
\sum w_i = 
\frac {1}  { \Tr (A_{i^\ast} ) +\Tr (B_{i^\ast} )}  
\]
This implies $O(\log (\ell+ m))$ iterations of binary decision problem, 

Let $n= \ell + m$. For 
 \begin{align}
& \Tr (A_i + B_i) \ge n^3 \Longrightarrow \max \Big ( \| A_i \|, \frac {\|B \|_k} k \Big ) \ge n^2 \\
& \Longrightarrow  w_i \le \frac 1 { n^2} \\
& \Longrightarrow \sum w_i 1 \big ( \Tr (A_i+ B_i ) \ge n^3 \big ) \le n \frac 1 {n^2} = \frac 1 n 
 \end{align}
 
 Thus removing $
 \begin{pmatrix} A_i & 0 \\0 & B_i \end{pmatrix}$ matrices with $\Tr (A_i + B_i) \ge n^3$ changes opt by less than $1/n$.    
 
 \subsection{Proof of Duality}

Primal covering 

Let $p^\ast : = \min \Tr (M) + \Tr (W)$ such that 
\[
\langle M, A_i \rangle, \langle W, B_i \rangle \ge 1, \quad \forall i \in [m]; \qquad M, W \succeq   0, \; M    \preceq \frac{ \Tr (M) } k I
\]
Dual Packing $d^ast := \max \sum W_i $ such that 
\[
\sum w_i  B_i \preceq I, \; \| \sum w_i A_i \|_k \le K,  \; w_i \ge 0
\]
Proof of duality: Conic Lagrangian 
\[
L(M, W, w, \Lambda, \phi) = \Tr (M) + \Tr (W) + \sum w_i (1- \langle M, A_i \rangle-
 \langle W, B_i \rangle) -  \langle \Lambda, M \rangle, \langle \phi,  W \rangle
 \]
for $w_i \ge 0, \forall i \in [m], \psi \succeq 0$ because PSD cone is self dual. Let 
\[
K := \Big \{ M | 0 \preceq M  \preceq \frac{ \Tr (M) } k I  \Big  \} 
\]
be a cone. Let $K^\ast$ be teh dual cone of $K$. Let $\Lambda \in K^\ast$. 

Thus we have 
\begin{align}
p^\ast : = &  \min_{M, W} \max_{w \ge 0, \Lambda \in K^\ast, \Psi \succeq 0}  L(M, W, w, \Lambda, \phi) \\
= & \min_{M, W} \max_{w \ge 0} \sum w_i + \max_{\Lambda \in K^\ast}
\langle I - \sum w_i A_i - \Lambda, M \rangle + \max_{ \Psi \succeq 0} 
\langle I - \sum w_i B_i - \Psi, W \rangle\\
\ge & d^\ast := \max_{w , \Lambda , \Psi } g(w, \Lambda, \phi) 
 \end{align} 
   where 
 \begin{align}
g(w, \Lambda, \phi) : 
= & \min_{M, W} \sum w_i + 
\langle I - \sum w_i A_i - \Lambda, M \rangle - \langle I -  \sum w_i B_i - \Psi, W \rangle \\
= & \begin{cases}  \sum w_i & \text { if }  
I - \sum w_i A_i - \Lambda = 0, \;    I - \sum w_i B_i - \Psi=0 \text{ and } w_i  \ge 0 \\
= \infty & \text{ otherwise} 
\end{cases}
 \end{align} 

The dual 
\[
 d^\ast : =  \max \sum w_i 
 \] 
 such that 
 \[
 w_i  \ge 0, \forall i \in [m], \; I - \sum w_i A_i - \Lambda = 0, \;    I - \sum w_i B_i - \Psi=0, 
   \Psi \ge 0, \text{ and } \Lambda \in K^\ast
\]
is equivalent to 
\[
 \max \sum w_i 
 \] 
 such that 
 \[
 w_i  \ge 0, \forall i \in [m], \;   \sum w_i B_i  \preceq I, \;
I - \sum w_i A_i \in K^\ast.
\]

Consider $K^\ast$. By definition of dual cone, 
\begin{align}
\forall M \in K^\ast, &  \; \langle I , M  \rangle -
\langle  \sum w_i A_i , M \rangle \ge 0  \\
\Longleftrightarrow & \Tr (M) = \max_{M \in K}  \langle  \sum w_i A_i , M \rangle \ge 0 \\
\Longleftrightarrow & \Tr (M) - \frac { \Tr (M) } k \|  \sum w_i A_i \|_k \ge 0 \\
 \Longleftrightarrow & \|  \sum w_i A_i \|_k \le  k 
 \end{align} 
 Thus 
 \[
 d^\ast : =  \max \sum w_i 
 \] 
 such that 
 \[
 w_i  \ge 0, \forall i \in [m], \;     \sum w_i B_i \preceq I, \; \|  \sum w_i A_i \|_k \le  k 
  \]

\qed

==> content/appformal.tex <==
\section{Formal Error Analysis}
In the ensuing sections we prove that an appropriate binary search over the primal dual solver yields an efficient approximation of the min max optimization.  We then prove that the approximate gaurantees suffice for the operation of our list decoding algorithm. 

\subsection{Approximating Min-Max Optimization via Primal Dual SDP}

\paragraph{Notation: } For this section we will fix the shift parameter $\nu$, weight upper bound parameter $\hat{w}$, and fix the $k$-norm hence dropping all three from notational subscripts.  Let SDP-OPT$(\theta)$ be the optimum of primal dual SDP for the packing/covering parameter $\theta$.  SDP-Solver$(\theta,\eps)$ is the procedure that approximately finds SDP-OPT$(\theta)$ up to a multiplicative error of $\eps$.  Let $SDP_P(\theta)$ and $SDP_D(\theta)$ denote the set of primal and dual feasible sets of (will replace when section is done). Let Min-MaxOPT$(\tau,k)$ be the optimum of the convex concave optimization at $\tau \in [\frac{1}{2}, \frac{1}{1+\eps}]$ and $k \in \Z^+$.  Let BinarySearch$(\tau,\eps)$ be the procedure that solves for Min-MaxOPT$(\tau,k)$.   Let $f(w,M) := \langle M, \sum_{i=1}^N w_iX_iX_i^T \rangle$.  Let $\Phi(\gamma) := \{w \in \R^N | 0 \leq w_i \leq \hat{w_i} \text{ } \forall i \in [N] \text{ and } \norm{w}_1 = \gamma\}$ denote a set of weights. 

Algorithm Description:  For a target Min-Max optimum $\tau \in [\frac{1}{2}, \frac{1}{1+\eps}]$ and SDP approximation parameter $\eps \in [0,\frac{1}{2}]$, BinarySearch$(\tau,\eps)$ outputs a triple $(\theta^*,M^*,w^*)$ where $\theta^* \in \R^+$ is an approximate Min-MaxOPT$(\tau,k)$, $M^* \in \R^{d \times d}$ is an approximately primal optimal point, and $w^* \in \R^{N}$ is an approximately dual optimal point.  These notions will be made precise later.  BinarySearch$(\tau,\eps)$ calls SDP-Solver$(\theta,\eps)$  for $\theta \in [\frac{1}{k}, \frac{dk}{\alpha}]$ until a $\theta^*$ is found satisfying SDP-OPT$(\theta^*) \in [\tau(1-\eps),\tau(1+\eps)]$.  We prove that this can be done in no more than $O(\log(\frac{dk^2}{\eps\alpha}))$ calls to SDP-Solver$(\theta,\eps)$ see \ref{lem:binarysearch}.  SDP-Solver$(\theta^*,\eps)$ also outputs a pair of primal $(\widetilde{M},\widetilde y)$ and dual $\widetilde w$ variables that are $SDP_P(\theta)$ and $SDP_D(\theta)$ feasible respectively and approximately attain the target optimum $\tau$.  That is to say $Tr(\widetilde{M}) + \norm{\widetilde{y}}_1 \leq \tau(1+\eps)$ and $\sum_{i=1}^N \widetilde{w_i} \geq \tau(1 - \eps)$ (See SDP-Solver$(\theta,\eps)$ guarantees).  Then for $M^\ast = \frac{\widetilde{M}}{\Tr (\widetilde{M})}$ and $w^\ast := \tau(1-\eps)\frac{\widetilde{w}}{\norm{w}_1}$, we have $M^* \in S_k$ and $w^* \in \Phi(\tau(1-\eps))$. Furthermore,  $(\theta, M^*, w^*)$ satisfies $\max_{M \in S_k} f(w^*,M) \leq \theta \leq \min_{w \in \Phi(\tau(1 + \eps))} f(w,M^*)$.  For the proof of this last statement see \ref{lem:approxminmax}.  Formalizing this discussion, we have   

\begin{lemma} \label{lem:approxmain}(Binary Search Guarantee)
For a target Min-Max optimum $\tau \in [\frac{1}{2}, \frac{1}{1+\eps}]$ and SDP approximation parameter $\eps \in [0,\frac{1}{2}]$, BinarySearch$(\tau,\eps)$ outputs a triple $(\theta^*,M^*,w^*)$ satisfying SDP-OPT$(\theta^*) \in [\tau(1-\eps),\tau(1+\eps)]$ and  $\max_{M \in \mathcal{F}_k} f(w^*,M) \leq \theta \leq \min_{w \in \Phi(\tau(1 + \eps))} f(w,M^*)$.  Furthermore, this can be done with no more than $O(\log(\frac{dk^2}{\eps\alpha}))$ calls to SDP-Solver$(\theta,\eps)$
\end{lemma}

\begin{proof}
    The proof follows directly by the algorithm description and \ref{lem:approxminmax} and \ref{lem:binarysearch}.  
\end{proof}

\begin{lemma} \label{lem:approxminmax} (Approximate Min-Max Optimization)
Let $(\widetilde{M},\widetilde{y})$ and $\widetilde{w}$ be a pair of primal dual feasible solutions to $SDP_P(\theta)$ and $SDP_D(\theta)$ approximately attaining an optimum $\tau := $ SDP-OPT$(\theta)$.  That is to say $Tr(\widetilde{M}) + \norm{\widetilde{y}}_1 \leq \tau(1+\eps)$ and $\sum_{i=1}^N \widetilde{w_i} \geq \tau(1 - \eps)$.  Then for $M^\ast = \frac{\widetilde{M}}{\Tr (\widetilde{M})}$ and $w^\ast := \tau(1-\eps)\frac{\widetilde{w}}{\norm{w}_1}$, we have $M^* \in S_k$ and $w^* \in \Phi(\tau(1-\eps))$. Furthermore,  $(\theta, M^*, w^*)$ satisfies $\max_{M \in S_k} f(w^*,M) \leq \theta \leq \min_{w \in \Phi(\tau(1 + \eps))} f(w,M^*)$
\end{lemma}
\begin{remark}
 This is the sense in which $M^\ast, w^\ast$ are approximate maximin and minimax solutions of the convex concave optimization.  The $\eps$ approximation parameter of the SDP solver manifests itself as an approximation in the weight constraints.  We will use the relation $\max_{M \in S_k} f(w^*,M) \leq \theta \leq \min_{w \in \Phi(\tau(1 + \eps))} f(w,M^*)$ to provide all formal guarantees for our list decoding algorithm.        
\end{remark}
\begin{proof} We run through first the analysis of the primal $M^*$ and then the dual $w^*$.   
\paragraph{Primal: }Consider the primal covering solution $(\widetilde{M}, \widetilde{y})$ satisfying.   
\[
\Tr (\widetilde{M}) + \sum_{i=1}^N \widetilde{y}_i \leq \tau(1 + \eps).
\]
Using the constraints $ \frac 1 \theta \langle \widetilde{M},   X_i X_i^T \rangle + \frac { \widetilde{y}_i} { \hat w_i} \ge 1$
and $\widetilde{y}_i \ge 0$ in SDP-P$(\theta)$, we substitute $\widetilde{y}_i \geq \hat w_i \max \Big ( 1 -  \frac 1 \theta \langle \widetilde{M},   X_i X_i^T \rangle, 
0 \Big )$ to obtain  
\[
\Tr (\widetilde{M}) + \sum_{i=1}^N \hat w_i \max \Big ( 1 -  \frac 1 \theta \langle \widetilde{M},   X_i X_i^T \rangle, 
0 \Big ) \le \tau(1+\eps).
\]
Let $S  = \{ i \in [N]| \langle \widetilde{M},   X_i X_i^T \rangle  \le \theta \}$. Then we rewrite the above expression as
\[
\Tr (\widetilde{M}) +  \sum_{i \in S}  \hat w_i -\frac 1 \theta   \sum_{i \in S}   \hat w_i \langle \widetilde{M},   X_i X_i^T \rangle \le \tau(1 + \eps)\\
\]
Further rearranging we obtain 
\begin{align}\label{eq:app1}
& \theta \Tr (\widetilde{M}) + \theta \Big (\sum_{i \in S}  \hat w_i - \tau(1+\eps) \Big ) \le 
    \sum_{i \in S}   \hat w_i \langle \widetilde{M},   X_i X_i^T \rangle
\end{align}
Now consider the following two cases. 

\paragraph{Primal Case 1:} Firstly, consider the case where $ \sum_{i \in S}   \hat w_i > \tau(1+\eps)$.  Then for $f^\ast = \min_{w \in \Phi(\tau(1+\eps))} f(w,\widetilde{M})$, let $w'$ be a set of weight such that $f(w',\widetilde{M}) = f^\ast $.  Since $w'$ selects the smallest $\tau(1+\eps)$ weighting of the collection $\{\langle \widetilde{M},X_iX_i^T\rangle\}_{i=1}^N$, we have by the definition of $S$ and the assumption $ \sum_{i \in S}   \hat w_i > \tau(1+\eps)$, that $w'$  is $0$ for $i \in S^c$ or equivalently $\sum_{i \in S} w^\prime_i=\tau(1+\eps)$.  
Thus, we have 
\[\sum_{i \in S}   \hat w_i \langle \widetilde{M},   X_i X_i^T \rangle 
= \sum_{i \in S}  ( \hat w_i- w^\prime_i)  \langle \widetilde{M},   X_i X_i^T \rangle +  \sum_{i =1}^N 
  w^\prime_i \langle \widetilde{M},   X_i X_i^T \rangle .
\]
Now by the definition of $S$, we upper bound the above expression by  
\[
\le  \theta  \sum_{i \in S}  ( \hat w_i- w^\prime_i)  +  \sum_{i =1}^N 
  w^\prime_i \langle \widetilde{M},   X_i X_i^T \rangle = \theta \Big (\sum_{i \in S}   \hat w_i- \tau(1+\eps) \Big )  +  \sum_{i =1}^N 
  w^\prime_i \langle \widetilde{M},   X_i X_i^T \rangle 
\]
Where the equality holds by the fact $\sum_{i \in S}  w^\prime_i = \tau(1+\eps) $. Now, plugging the upper bound back into \eqref{eq:app1} we obtain
\[
 \theta \Tr (\widetilde{M})+  \theta \Big (\sum_{i \in S}   \hat w_i- \tau(1+\eps) \Big )  
 \le \theta \Big (\sum_{i \in S}   \hat w_i- \tau(1+\eps) \Big ) +   \sum_{i =1}^N 
  w^\prime_i \langle \widetilde{M},   X_i X_i^T \rangle 
\]
Subtracting $ \theta \Big (\sum_{i \in S}   \hat w_i- \tau(1+\eps) \Big ) $ from both sides, 
we obtain $ \theta \Tr (\widetilde{M})
 \le  \sum_{i =1}^N 
  w^\prime_i \langle \widetilde{M},   X_i X_i^T \rangle$. Finally, dividing through by $\Tr (\widetilde{M})$ we obtain, 
$\theta \le  \sum_{i =1}^N 
  w^\prime_i \langle M^\ast , X_i X_i^T \rangle = f(w',M^*)$.  By the definition of $w'$ we know that $f(w',M^*) = \min_{w \in \Phi(\tau(1+\eps))} f(w,M^*)$ which concludes our proof of $\theta \leq \min_{w \in \Phi(\tau(1+\eps))} f(w,M^*)$ for case 1.    

\paragraph{Primal Case 2:} For the case where $\sum_{i \in S}   \hat w_i \le \tau(1+\eps)$, by the definition of $S$ we have 
$w^\prime_i = \hat w_i$ for all $i \in S$. Therefore, the right hand side of \eqref{eq:app1} is equal to 
\begin{align} 
 \sum_{i \in S}   \hat w_i  \langle \widetilde{M},   X_i X_i^T \rangle 
=\sum_{i \in S}    w^\prime_i  \langle \widetilde{M},   X_i X_i^T \rangle = \sum_{i =1}^N    w^\prime_i  \langle \widetilde{M},   X_i X_i^T \rangle 
-\sum_{i \in S^c}    w^\prime_i  \langle \widetilde{M},   X_i X_i^T \rangle
\end{align}
By definition of $S$, we upper bound by  
\begin{align}\label{eq:app2}
\le \sum_{i =1}^N    w^\prime_i  \langle \widetilde{M},   X_i X_i^T \rangle 
-\sum_{i \in S^c}    w^\prime_i  \theta 
\end{align}
Now noting that $\sum_{i \in S^c}    w^\prime_i = \sum_{i =1}^N   \big  (w^\prime_i  - w^\prime_i 1(i \in S) \big )
= \sum_{i =1}^N   \big  (w^\prime_i  - \hat  w_i 1(i \in S) \big )= \tau(1+\eps)-\sum_{i \in S}    \hat w_i$
Plugging this equality into \eqref{eq:app2}, we obtain 
\[
\eqref{eq:app2} = \sum_{i =1}^N    w^\prime_i  \langle M,   X_i X_i^T \rangle   -  \Big (1- \sum_{i \in S}   \hat w_i \Big ) p
\]
Plugging this upper bound into the right hand side of \eqref{eq:app1} we obtain
\begin{align}
\theta \Tr (\widetilde{M})+  \theta \Big (\sum_{i \in S}   \hat w_i- \tau(1+\eps) \Big )  
 \le \sum_{i =1}^N    w^\prime_i  \langle \widetilde{M},   X_i X_i^T \rangle   -  \Big (\tau(1+\eps)- \sum_{i \in S}   \hat w_i \Big ) \theta
 \end{align}
 Canceling terms on both sides we obtain
 $\theta \Tr (\widetilde{M})
 \le \sum_{i =1}^N    w^\prime_i  \langle \widetilde{M},   X_i X_i^T \rangle$.  
 Now dividing through by $\Tr (\widetilde{M})$ we conclude 
 $
\theta
 \le \sum_{i =1}^N    w^\prime_i  \langle M^\ast ,   X_i X_i^T \rangle  $
 Once again, by the definition of $w'$ we have 
 $\min_{w \in \Phi(\tau(1+\eps))} f(w,M^*)\ge \theta$ which concludes our treatment of the primal $M^*$ for both cases. 
 
\paragraph{Dual: } Now consider the dual solution $\widetilde{w}$ satisfying $SDP_D(\theta)$. We have $\widetilde{w}$ satisfying  
 $\norm{\widetilde{w}}_1 \geq \tau(1-\eps)$ and $\max_{M \in S_k}f(\widetilde{w},M) \leq \theta$ which we use to conclude 
\begin{align}
    \max_{M \in S_k} f(w^*,M) =  \frac{\tau(1-\eps)}{\norm{w}_1}\max_{M \in S_k}f(\widetilde{w},M) \leq \frac{\tau(1-\eps)}{\norm{w}_1}\theta \leq \theta
\end{align}
This concludes the proof of $\max_{M \in S_k} f(w^*,M) \leq \theta \leq \min_{w \in \Phi(\tau(1 + \eps))} f(w,M^*)$.    
\end{proof}

We prove that the binary search procedure terminates in $O(\log(d))$ iterations
\begin{lemma} \label{lem:binarysearch}
     For any $\eps \in [0,\frac{1}{2}]$ and for any $\tau \in [\frac{1}{2},\frac{1}{1+\eps}]$, BinarySearch$(\tau,\eps)$ outputs a triple $(\theta^*, M^*, w^*)$.    such that SDP-OPT$(\theta^*) \in [\tau(1 - \eps),\tau(1 + \eps)]$  via no more than $O(\log(\frac{dk^2}{\eps\alpha})$ iterations of binary search over $\theta$ in the interval $[\frac{1}{k},\frac{dk}{\alpha}]$.      
\end{lemma}
\begin{proof}
    To enable binary search it suffices to exhibit upper and lower bounds of $[\frac{1}{k},\frac{dk}{\alpha}]$ on the range of $\theta$; demonstrate that SDP-OPT$(\theta)$ is monotonically increasing; and finally prove that SDP-OPT$(\theta)$ takes values in $[\tau(1 - \eps), \tau(1+\eps)]$ over an interval of $\theta \in \R^+$ of length larger than $\frac{\eps}{k}$.  Given all three of the above facts, a binary search over the interval $[\frac{1}{k},\frac{dk}{\alpha}]$ would output a $\theta^*$ such that $SDP(\theta^*) \in [\tau(1 - \eps),\tau(1+\eps)]$ in no more than $O(\log(\frac{dk^2}{\eps\alpha})$ iterations.  
    
    First we prove $\theta$ is upper bounded by $\frac{dk}{\alpha}$.  By the naive warm start algorithm, all points lie within $O(\sqrt{d})$ of the origin.  Thus we can naively bound the k-norm of $\frac{1}{\alpha N}\sum_{i=1}^N X_iX_i^T$ by $$\norm{\frac{1}{\alpha N}\sum_{i=1}^N X_iX_i^T}^*_k \leq k\max_{v \in S^{d-1}} \frac{1}{\alpha N}\sum_{i=1}^N \langle X_i,v\rangle^2 \leq \frac{dk}{\alpha}$$   
    
    
    On the other hand, we can lower bound the value of $\theta$ by $\frac{1}{k}$.  Assuming the contrary. If SDP-OPT$(\theta) \geq \tau$ for $\theta \leq \frac{1}{k}$, it implies $\norm{\sum_{i=1}^N w_i X_iX_i^T}^*_k \leq 1$ for a $w \in \Phi(\tau)$ which terminates the algorithm by lemma \ref{lem:basecase} for $\tau \in [\frac{1}{2}, \frac{1}{1+\eps}]$.
    
     Next we prove that SDP-OPT$(\theta)$ is monotonic in $\theta$.  Let $D(\theta) := \{w \in \R^N| w \text{ satisfies } SDP_D(\theta)\}$.  Noting that $D(\theta_1) \subseteq D(\theta_2)$ for any $\theta_1 < \theta_2 \in \R^+$ we conclude SDP-OPT$(\theta)$is monotonic in $\theta$.   
     
     Finally, for $w_2 \in D(\theta_2)$ attaining SDP-OPT$(\theta_2)$, we have $\frac{\theta_1}{\theta_2}w_2 \in D(\theta_1)$.  Therefore SDP-OPT$(\theta_1) \geq \frac{\theta_1}{\theta_2}\norm{w_2}_1 = \frac{\theta_1}{\theta_2}$SDP-OPT$(\theta_2)$.  For the special case of SDP-OPT$(\theta_2) = \tau$ we obtain SDP-OPT$(\theta_1) \geq \frac{\theta_1}{\theta_2}\tau$ which implies the interval of values of $\theta$ over which SDP-OPT$(\theta) \in [\tau(1 - \eps),\tau]$ is greater than $\eps\theta_2 \geq \frac{\eps}{k}$ where we use the fact that $\theta_2 \geq \frac{1}{k}$.    
\end{proof}


==> content/notes.tex <==
\section{Rough notes}

\paragraph{Problem statement.}  Let $X\subseteq\R^d$ such that $|X|=n$, let $S\subseteq X$ such that $|S|=\alpha n$, let $\mu \coloneqq \E_{\bx\sim S}\bx$, and finally assume $\E_{\bx\sim S}(\bx-\mu)(\bx-\mu)^{\Transp}\psdle\Id$.  The goal is to output a collection of points $L$ of size $O(1/\alpha)$ such that $d(\mu,L)\le O\left(\sqrt{1/\alpha}\right)$.

\paragraph{Min-max game.}  Given a ``weight budget'' $b_x$ per point $x\in X$, a ``guess'' $\nu\in\R^d$ and a parameter $C\ge 0$, we define
\begin{align*}
    \Cost(\nu, X, b, C) \coloneqq \min_{\substack{0\le w_x\le b_x \\ \sum_{x\in X} w_x = 1}} \max_{\substack{0 \psdle M\psdle C\cdot\Id\\ \Tr(M)=1}} \left\langle M, \sum_{x\in X} w_x (x - \nu) (x - \nu)^{\transp} \right \rangle.
\end{align*}
Key to our result is an algorithm to efficiently\snote{Be more precise; state runtime dependence on $\eps$.} approximate $\Cost(v,X,b,C)$ as well as produce weights $w^*$, and a matrix $M^*$ that approximately solve the program above.  More precisely, they satisfy the conditions\snote{Check!!  I half made these up}
\[
    \max_{\substack{0 \psdle M\psdle C\cdot\Id\\ \Tr(M)=1}} \left\langle M, \sum_{x\in X}w_x^*(x-\nu)(x-\nu)^{\transp} \right\rangle \le (1+\eps)\Cost(\nu, X, b, C)
\]
and
\[
    \left\langle M^*, \sum_{x\in X}w_x^*(x-\nu)(x-\nu)^{\transp} \right\rangle \ge (1-\eps)\max_{\substack{0 \psdle M\psdle C\cdot\Id\\ \Tr(M)=1}} \left\langle M, \sum_{x\in X}w_x^*(x-\nu)(x-\nu)^{\transp} \right\rangle.
\]
Henceforth, we use $\Wts(\nu,X,b,C)$ to refer to $w^*$ and $\Advice(\nu,X,b,C)$ to refer to $M^*$.





\paragraph{Algorithm \textsf{OutputCluster}.}

We begin by stating fixed constants in our algorithm.\\
\noindent $k = 1/\alpha,~\ell = 10^{10}\cdot k,~r^2 = 10^{10}\cdot\ell,~s= 10^5\cdot\ell,~p=\wt{O}(k)$.\snote{Pick $p$ more precisely}
\begin{align*}
    \text{Input: } \quad  & \text{ Set of points  $X$, weight budget $b$}\\
    \theta^{(0)} &= \infty, t=1, \nu^{(0)} = 0 \\
    \theta^{(1)} &= \Cost(\nu^{(0)},X,b,1/\ell)\\
    M^{(1)} &= \Advice(\nu^{(0)},X,b,1/\ell)\\
    w^{(1)} &= \Wts(\nu^{(0)},X,b,1/\ell)\\
    \text{While}, \quad & \theta^{(t)}  \le 0.99\cdot \theta^{(t-1)}\\
    & V^{(t)}  = \SVD_\ell (M^{(t)}), \quad Y^{(t)} = \{\nu^{(t-1)}+\Pi_{V^{(t)}}(x-\nu^{(t-1)}):x\in X\} \\
    & \text{Pick $\by_1,\dots,\by_p$ independently and uniformly from $Y^{(t)}$}  \\
    & \theta^{(t+1)}  = \min_{j\in[p]} \Cost(\by_j,X,b,1/\ell) \\
    & \nu^{(t+1)} = \argmin_{\by_j\in\{\by_1,\dots,\by_p\}} \Cost(\by_j,X,b,1/\ell) \\
    & M^{(t+1)} = \Advice(\nu^{(t+1)},X,b,1/\ell) \\
    & w^{(t+1)} = \Wts(\nu^{(t+1)},X,b,1/\ell)\\
    & t=t+1 \\
    \text{end} \quad & \\
    & T=t-1 \\
    & V = \SVD_\ell\left(\sum_{x\in X} w_x^{(T)} \left(x - \nu^{(T)}\right)\left(x - \nu^{(T)}\right)^{\transp} \right) \\
    & \text{Let $x_1,\dots,x_n$ be an ordering of $X$ so that }\\
    &\left\|\Pi_V(x_1-\nu^{(T)})\right\| \le \left\|\Pi_V(x_2-\nu^{(T)})\right\| \le \ldots \left\|\Pi_V(x_n-\nu^{(T)})\right\| \\
    \text{Output:}   \quad & (\nu,w) \text{where $\nu\coloneqq\nu^{(T)}$ and $w$ is the lowest $0.1$ fraction $w^{(T)}$.}
\end{align*}
\snote{explain what this means}


{\bf Algorithm  \textsf{OutputList}.} 

\begin{align*}
    \text{Input:} \quad  & \text{ Set of points  $X$,   fraction $\alpha$}\\
    & \forall x \in X:~ b_x = \frac{2}{\alpha n}, \;  L = \{ \} \\
    \text{While}, \quad & \sum_{x\in X}  b_x  \ge 1\\
    & (\nu, w) =  \textsf{OutputCluster}(X, b)\\
    & L = L\cup\{\nu\} \\
    & b =  b - w \\
  \text{end} \quad &\\
  \text{Output:} \quad & L
 \end{align*}


\begin{lemma}   \label{lem:progress-0.75}
    Let $(\nu,w)$ be the output of the algorithm \textsf{OutputCluster}\snote{Figure out the algbox stuff and number this} on input $X$ and $b$, and let
    \[
        \wt{\mu}\coloneqq \sum_{x\in S}\frac{b_x}{\sum_{y\in S}b_y} x.
    \]
    Suppose $\sum_{x\in S}b_x\ge 1$, then $\theta^{(T)} \le \frac{0.75\|\wt{\mu}-\nu\|^2}{\ell}$.\snote{Check}
\end{lemma}
\snote{Insert proof}


\begin{lemma} 
\textsf{OutputCluster}\snote{Number this} when given input $X$ and $b$ such that $\sum_{x\in S} b_x  \ge 1$ and for all $x\in X$, $b_x\le  \frac{2}{\alpha n}$, produces 
$(\nu, w)$ as output satisfying 
\begin{enumerate}
\item $\|\nu - \mu\| \le r$ or
\item $\sum_{i \in S} w_x \le \frac{1}{10^3k}$.
\end{enumerate}
\end{lemma} 

\begin{proof} 
Assume $\|\nu - \mu\| > r$, and define
\begin{align*}
    \theta^\ast &\coloneqq \Cost(\nu,X,b,1/\ell)\\
    \wt{\mu} &\coloneqq \sum_{x \in S}\frac{b_x}{\sum_{y \in S} b_y} x\\
    \wt{\Sigma} &\coloneqq \sum_{x\in X}w_x(x-\nu)(x-\nu)^{\transp}
\end{align*}
First, we note that from \pref{lem:progress-0.75}, $\theta^\ast \le \frac{0.75 \|\nu-\wt{\mu}\|^2}{\ell}$.  Next, we observe that $\sigma_{\ell}\left(\wt{\Sigma}\right) \le \theta^*$.\snote{Justify.  Basically $\theta^*$ is the average of the first $\ell$ singular values.  Put justification in preliminaries}.  We also note that from \pref{lem:resilience}, $\|\mu-\wt{\mu}\|\le\sqrt{2}$, which means $\left|\|\wt{\mu}-\nu\|-\|\mu-\nu\|\right|\le \sqrt{2}$.  Combined with the fact that $\|\mu-\nu\|>r$, we can derive
\begin{align}   \label{eq:closeness-means}
    \|\mu-\nu\| \ge .99\|\wt{\mu}-\nu\|
\end{align}
Now, let $w_S =  \sum_{x \in S} w_x$.  If $w_S \le \frac 1 {10^3 k} $ we would be done so for the rest of the proof we assume $w_S\ge \frac{1}{10^3 k}$.

Let $V= \SVD_\ell\left(\wt{\Sigma}\right)$.  Let $\Pi_V$ be the projection onto the column space of $V$.  We now claim $\|\Pi_V(\mu-\nu) \| \ge 0.99 \|(\mu-\nu)\|$.  Suppose not, then $\|\Pi_V^\perp(\mu - \nu) \| \ge 0.01 \|\mu-\nu\|$.
Let $\vphi \coloneqq \frac{\Pi_V^\perp(\mu-\nu)}{\|\Pi_V^\perp(\mu-\nu)\|}$.  Then
\begin{align*}
    \vphi^{\transp}\wt{\Sigma}\vphi &= \sum_{x\in X} w_x \langle \vphi, x-\nu\rangle^2\\
    &\ge \sum_{x\in S} w_x \langle \vphi, x-\nu\rangle^2\\
    &= \sum_{x\in S} w_x \langle \vphi, x-\mu + \mu-\nu\rangle^2\\
    &= \sum_{x\in S}w_x \left(\langle\vphi,x-\mu\rangle^2 + 2\langle\vphi, x-\mu\rangle\langle\vphi,\mu-\nu\rangle + \langle\vphi,\mu-\nu\rangle^2\right)\\
    &= \sum_{x\in S}w_x\left(\langle\vphi,x-\mu\rangle + \langle\vphi,\mu-\nu\rangle\right)^2\\
    &= w_S \sum_{x\in S}\frac{w_x}{w_S}\left(\langle\vphi,x-\mu\rangle + \left\|\Pi_V^{\perp}(\mu-\nu)\right\|\right)^2  \numberthis \label{eq:to-lower-bound}
\end{align*}
Let $\by$ be sampled from $S$ with probability $\frac{w_x}{w_S}$.  First we show that $\E\left[\langle\vphi, \by-\mu \rangle^2\right]$ is bounded by $\frac{2000}{\alpha}$.  To see this, we first write
\begin{align*}
    \E\left[\langle\vphi, \by-\mu \rangle^2\right] &= \sum_{x\in S}\frac{w_x}{w_S}\langle \vphi, x-\mu\rangle^2.
\end{align*}
Since each $w_x\le\frac{2}{\alpha n}$, and $w_S\ge\frac{\alpha}{1000}$, the RHS of the above can be upper bounded by
\[
    \sum_{x\in S}\frac{2000}{\alpha^2 n}\langle \vphi, x-\mu\rangle^2 = \frac{2000}{\alpha} \sum_{x\in S}\frac{1}{\alpha n}\langle \vphi, x-\mu\rangle^2.
\]
Since the uniform distribution on $S$ has covariance spectrally bounded by $1$, we indeed have
\[
    \E\left[\langle\vphi, \by-\mu \rangle^2\right] \le \frac{2000}{\alpha}.
\]
By Markov's inequality, 
\[
    \Pr[|\langle\vphi,\by-\mu\rangle| > 10^{12}\sqrt{k}] \le \frac{\sqrt{2000k}}{10^{12}\sqrt{k}} \le \frac{1}{10^8}.
\]
Since $\|\mu-\nu\| \ge 10^{15}\sqrt{k}$, $\|\Pi_V^{\perp}(\mu-\nu)\| \ge 10^{13}\sqrt{k}$, the above implies that
\[
    \Pr\left[\langle\vphi,\by-\mu\rangle < -0.1\left\|\Pi_V^{\perp}(\mu-\nu)\right\|\right] \le \frac{1}{10^8}
\]
This means we can lower bound \pref{eq:to-lower-bound} by
\begin{align*}
    w_S \left(1-\frac{1}{10^8}\right)\cdot\left(0.9\left\|\Pi_V^{\perp}(\mu-\nu)\right\|\right)^2 &\ge \frac{\|\mu-\nu\|^2}{10^9k}\\
    &\ge 10\frac{\|\mu-\nu\|^2}{\ell}\\
    &\ge 9\frac{\|\wt{\mu}-\nu\|^2}{\ell} &\text{from \pref{eq:closeness-means}}\\
    &> \theta^*.
\end{align*}
In short, $\vphi^{\transp}\wt{\Sigma}\vphi>\theta^*$.  On the other hand since $\vphi$ is a unit vector in the space orthogonal to $V$ it must be the case that $\vphi^{\transp}\wt{\Sigma}\vphi\le\sigma_{\ell+1}\left(\wt{\Sigma}\right)\le\theta^*$, which is a contradiction.  Thus, the assumption that $\|\Pi_V^{\perp}(\mu-\nu)\|\ge.01\|\mu-\nu\|$ is flawed and $\|\Pi_V(\mu-\nu)\|\ge.99\|\mu-\nu\|$.

Next, observe that
\[
    \trace\left(\Pi_V\wt{\Sigma}\Pi_V\right) = \sum_{i=1}^\ell \sigma_i\left(\wt{\Sigma}\right) = \ell\cdot\theta^{\ast} \le .75\|\nu-\wt{\mu}\|^2
\]
It is also the case that
\[
    \trace\left(\Pi_V\wt{\Sigma}\Pi_V\right) = \sum_{x\in X}w_x\left\|\Pi_V(x-\nu)\right\|^2.
\]
Thus, if $\bx$ is sampled from $X$ with probability $w_{\bx}$ then
\[
    \E\|\Pi_V(\bx-\nu)\|^2 \le .75\|\nu-\wt{\mu}\|^2 \le .76\|\nu-\mu\|^2.
\]
% \snote{justify the inequality from .75 to .76 and going from $\wt{\mu}$ to $\mu$.}
and thus by Markov's inequality,
\[
    \Pr\left[\|\Pi_V(\bx-\nu)\|^2 \le .85\|\nu-\wt{\mu}\|^2\right] \ge 1 - \frac{.75}{.85} \ge .1.
\]
Now, let $\bx'$ be uniformly sampled from $S$.
\begin{align*}
    \|\Pi_V(\bx'-\nu)\|^2 &= \langle \Pi_V(\bx'-\mu+\mu-\nu),\bx'-\mu+\mu-\nu\rangle\\
    &= \langle\bx'-\mu,\Pi_V(\bx'-\mu)\rangle + 2\langle\Pi_V(\mu-\nu),\bx'-\mu\rangle + \langle\Pi_V(\mu-\nu), \mu-\nu\rangle\\
    &\ge .99^2\|\mu-\nu\|^2 - 2|\langle\Pi_V(\mu-\nu),\bx'-\mu\rangle|\numberthis\label{eq:proj-mean-guess-diff}
\end{align*}
$\langle\Pi_V(\mu-\nu),\bx'-\mu\rangle$ is a zero mean random variable with variance bounded by $\|\Pi_V(\mu-\nu)\|^2$.  By Chebyshev's inequality,
\[
    \Pr[|\langle\Pi(\mu-\nu),\bx'-\mu\rangle| > t\|\mu-\nu\|] \le \frac{1}{t^2}.
\]
By setting $t = .01\|\mu-\nu\|$, we know that \pref{eq:proj-mean-guess-diff} is lower bounded by
\[
    .99^2\|\mu-\nu\|^2 - .02\|\mu-\nu\|^2 \ge .96\|\mu-\nu\|^2
\]
except with probability $\frac{1}{10^{-4}\|\mu-\nu\|^2}\le\frac{1}{10^{-4}r^2}\le\frac{1}{10^{16}k}$.

Since each $w_x$ is bounded by $\frac{2}{\alpha n}$,
\[
    w_S = \sum_{x\in S} w_x \le \frac{2}{10^{16}k},
\]
which contradicts the assumption that $w_S\ge\frac{1}{10^3k}$.
\end{proof}

\begin{comment}
COMPLETE THIS.
\begin{proof}
\newpage

\begin{align} 
    v^T \tilde \Sigma v & \ge 
    \sum_{i \in Y} \tilde \omega_i   \langle \mu, X_i - x  \rangle^2 \\ 
    &= \sum_{i \in Y} 
    \tilde \omega_i  \Big (  \langle \mu, X_i - \mu^\ast  \rangle^2- 2 \langle \mu, X_i -\mu^\ast  \rangle  \langle \mu, \mu^\ast -x \rangle 
    +  \langle \mu, x-  \mu^\ast  \rangle^2 \Big ) \\
    &  \ge  \sum_{i \in Y} 
    \tilde \omega_i  \Big (  0.99 \langle \mu, x- \mu^\ast  \rangle^2 - 
    100   \langle \mu, X_i-  \mu^\ast  \rangle^2 \Big ) \\
    \ge 10^{-6} \| x -  \mu^\ast \|^2 \ge \frac { \theta^\ast} \ell 
\end{align}
which is a contraction. Note by Markov's inequality, 
\[
\sum_{i: \| P_v ( X_i - x) \|^2 \le 0.85 d^2   }  \tilde \omega_i \ge 1 - \frac { 0.75} { 0.85} \ge 0.1. 
\]
For $i \in Y$, let $ \omega  = \frac { P_v ( X_i - x ) }   { \| P_v^\perp ( X_i - x ) \|}$. 
\begin{align} 
\| P_v ( X_i - x) \|^2 & \ge  \langle \omega, X_i - x  \rangle^2 \\
& \ge  \langle \omega, x - \mu^\ast   \rangle^2 - 2   \langle \omega, x - \mu^\ast   \rangle \langle \omega, X_i - \mu^\ast   \rangle
+  \langle \omega, X_i - \mu^\ast   \rangle^2 \\
& \ge 0.99 \langle \mu, x- \mu^\ast  \rangle^2 - 
   100   \langle \mu, X_i-  \mu^\ast  \rangle^2
\end{align} 
By Markov, we thus have 
\[
\mathbb P_{i \sim Y} \big ( \| P_v ( X_i - x )  \|^2 \le 0.85 d^2 \big ) \le \frac 1 { 10^6 k} .
\]
\end{proof} 


\[
k = 1/\alpha, \ell = 10^{10} k, r^2 = 10^{10} \ell, s= 10^5 \ell
\]
{\bf Algorithm-Output cluster} 


\begin{align} 
 \text{Input:} \quad  & \text{ Set of points  $(X_1, \ldots, X_n)$,   guess $x$}\\
&  \text{Weight budget $(\omega_1^\ast, \ldots, \omega_n^\ast)$.} \\
 \theta_0 & = \infty, x_0=x, t=1, \\
  \theta_1 & = \min_{ \substack{0 \le \omega  \le \omega_i^\ast\\ \sum  \omega_i = 1}} \max_{\substack{ \text{Tr} M = 1 \\ M \prec \frac 1 \ell I } } 
  \big \langle \sum \omega_i (X_i - x_0) (X_i - x_0) ^T,  M \big \rangle \\
 \text{While}, \quad & \theta_t  \le 0.99 \theta_{t-1}\\
 & V^{(t)}  = SVD_\ell ( M^{(t)}), \quad X_i^{(t)}= P_{V^{(t)}} (X_i) \\
 & \text{Pick}, \quad  \tilde O(k), Y_j^{(t)}  \text{randonly from  }, \quad X_i^{(t)}  \\
& \theta_{t+1}  = \min_j \min_{ \substack{0 \le \omega  \le \omega_i^\ast \\ \sum  \omega_i = 1}} \max_{\substack{ \text{Tr} M = 1 \\ M \prec \frac 1 \ell I } } 
  \big \langle \sum \omega_i (X_i - x_t) (X_i - x_t) ^T,  M \big \rangle \\
  & n_{t+1} = \argmin_j \min_{ \substack{0 \le \omega  \le \omega_i^\ast\\ \sum  \omega_i = 1}} \max_{\substack{ \text{Tr} M = 1 \\ M \prec \frac 1 \ell I } } 
  \big \langle \sum \omega_i (X_i - x_t) (X_i - x_t) ^T,  M \big \rangle\\
  & t=t+1 \\
 \text{end}, \quad & \\
 & T=t-1 \\
& V= SVD_\ell\big ( \sum \omega_i (X_i - x_t) (X_i - x_t) ^T \big ), \quad X_i^\ast= P_v(X_i - x_t) \\
 & \text{Let} \quad  i_1, \ldots i_n \text{ be} \; \le t,   \|X_{i_1}^\ast \| \le \|X_{i_1}^\ast \| \le \ldots \|X_{i_n}^\ast \| \\
 \text{Output:}   \quad & \text{ $x_t$ and the lowest $0.1$ fraction of the $\omega_i$}
\end{align}

\newpage 
{\bf Algorithm,  \quad Output list} 

\begin{align} 
 \text{Input:} \quad  & \text{ Set of points  $(X_1, \ldots, X_n)$,   fraction $\alpha$}\\
 & \omega_i^\ast = \frac 2 { \alpha n}, \; i \in [n], \;  \text{list } = \{ \} \\
 \text{While}, \quad & \sum  \omega_i^\ast  \ge 1\\
 &(x, \omega_i) =  \text{Output cluster} \; (X_1,  \omega_i^\ast)\\
 &\text{list} =  \{ \text{list}, x\} \\
 & \omega_i^\ast=  \omega_i^\ast -  \omega_i\\
  \text{end}, \quad &\\
  \text{Output: list} \quad &
 \end{align}

\begin{lemma} 
Output cluster when input $X_1, \ldots, X_n$ and $\sum  \omega_i^\ast  \ge 1$ and $\omega_i^\ast \le  \frac 2 { \alpha n}$, retrive 
$(x, \omega_i) $ satisfying 
\begin{enumerate}
\item $\| x - \mu^\ast \| \le \gamma$ or
\item $\sum_{i \in Y} \omega_i \le \frac 1 { 10^3 k} $
\end{enumerate}
\end{lemma} 

\begin{proof} 
Assume $\| x - \mu^\ast \| \ge  \gamma$.
\begin{align} 
  \theta^\ast  = \min_{ 0 \le \omega  \le \omega_i^\ast } \max_{\substack{ \text{Tr} M = 1 \\ M \prec \frac 1 \ell I } } 
  \big \langle \sum \omega_i (X_i - x) (X_i - x) ^T,  M \big \rangle 
\end{align}
$\tilde M, \tilde \omega_i$ corresponding arguments. 
\[
\tilde \mu = \frac {  \sum_{i \in Y} \omega_i^\ast X_i }{ \sum_{i \in Y} \omega_i^\ast  }, \quad d = \| x - \tilde \mu \| .
\]
\newpage 
we may assume $\theta^\ast \le 0.75 d^2$ as otherwise algorithm makes progress (we can get closer to plant). 
\[
\theta^\ast \le 0.75 d^2 \Longrightarrow \sigma_\ell \big (  \sum \omega_i (X_i - x) (X_i - x) ^T \big ) \le \frac { \theta^\ast} { \ell} .
\]
Let $\tilde \omega_Y =  \sum_{i \in Y} \omega_i  $.

If $\tilde \omega_Y \le  \frac 1 { 10^3 k} $, we are done. 

Let $\tilde \omega_Y \ge \frac 1 { 10^3 k} $ and $V= SVD_\ell  ( \tilde \Sigma  )$, where $\tilde \Sigma := \sum \omega_i (X_i - x) (X_i - x) ^T$.
We now claim $\| P_v ( \mu^\ast - x) \| \ge 0.99 \|  ( \mu^\ast - x) \|$. Assume the contrary, $\| P_v^\perp ( \mu^\ast - x) \| \ge 0.01 \|  ( \mu^\ast - x) \|$.
Let $\mu = \frac { P_v^\perp ( \mu^\ast - x) }   { \| P_v^\perp ( \mu^\ast - x) \|}$.
\begin{align} 
 v^T \tilde \Sigma v & \ge 
  \sum_{i \in Y} \tilde \omega_i   \langle \mu, X_i - x  \rangle^2 \\ 
  &  = \sum_{i \in Y} 
   \tilde \omega_i  \Big (  \langle \mu, X_i - \mu^\ast  \rangle^2- 2 \langle \mu, X_i -\mu^\ast  \rangle  \langle \mu, \mu^\ast -x \rangle 
   +  \langle \mu, x-  \mu^\ast  \rangle^2 \Big ) \\
    &  \ge  \sum_{i \in Y} 
   \tilde \omega_i  \Big (  0.99 \langle \mu, x- \mu^\ast  \rangle^2 - 
   100   \langle \mu, X_i-  \mu^\ast  \rangle^2 \Big ) \\
   \ge 10^{-6} \| x -  \mu^\ast \|^2 \ge \frac { \theta^\ast} \ell 
\end{align}
which is a contraction. Note by Markov's inequality, 
\[
\sum_{i: \| P_v ( X_i - x) \|^2 \le 0.85 d^2   }  \tilde \omega_i \ge 1 - \frac { 0.75} { 0.85} \ge 0.1. 
\]
For $i \in Y$, let $ \omega  = \frac { P_v ( X_i - x ) }   { \| P_v^\perp ( X_i - x ) \|}$. 
\begin{align} 
\| P_v ( X_i - x) \|^2 & \ge  \langle \omega, X_i - x  \rangle^2 \\
& \ge  \langle \omega, x - \mu^\ast   \rangle^2 - 2   \langle \omega, x - \mu^\ast   \rangle \langle \omega, X_i - \mu^\ast   \rangle
+  \langle \omega, X_i - \mu^\ast   \rangle^2 \\
& \ge 0.99 \langle \mu, x- \mu^\ast  \rangle^2 - 
   100   \langle \mu, X_i-  \mu^\ast  \rangle^2
\end{align} 
By Markov, we thus have 
\[
\mathbb P_{i \sim Y} \big ( \| P_v ( X_i - x )  \|^2 \le 0.85 d^2 \big ) \le \frac 1 { 10^6 k} .
\]
\end{proof} 

\end{comment}
\newcommand{\tr}{\text{Tr}}
\begin{comment}
\newpage 


\centerline{The regret bound} 

Fact: The Von Neumann entropy is 1-strongly continuous w.r.t. $\| \cdot \|$. 

Let $S= \{X:  X\ge 0, \Tr X =1, \|X \| \le 1/k \}$. 

Suppose one observes sequence of gain matrices 
\[
G_1, \ldots, G_T
\]
such that $\|G_i \| \le 1 \forall i \in [T]$.  Define 
\[
X_t = \argmin_{X \in S} \eta \sum_{i=1}^{t-1} \langle G_i, X \rangle - \Phi(X),
\]
where $\Phi(X) = \langle X, \log X \rangle$ is the Von-Neumann entropy. 

By theorem 5.2 in Hazun or  Theorem 4.3 is Bubeck 
\[
\text{Regret}_T = \max_{X \in S} \langle \sum_{i=1}^T G_i, X \rangle - \sum_{i=1}^T \langle G_i, X_i \rangle \le 2 \eta T + \frac { \log n } \eta
\]
as $\max_{X, Y \in S} \Phi(X) - \Phi(Y) \le \log \eta$. 

Taking $\eta = \sqrt { \frac {\log n } { 2 T} } $, we get 
\[
\text{Regret}_T \le  \sqrt {  2 T \log n }.
\]
Computing $X_t$ effectively. 


\begin{lemma} 
Let 
\[
X_t = \argmin_{X \in S} \eta \sum_{i=1}^{t-1} \langle G_i, X \rangle - \Phi(X).
\]
Then $X_t $ and  $\sum_{i=1}^{t-1}  G_i$ have the same eigenvector. 
\end{lemma} 

\begin{proof} 

 Let $X_t$ have eigenvalues $\sigma_1, \ldots \sigma_n$. Then 
\begin{align} 
& \eta \sum_{i=1}^{t-1} \langle G_i, X_t  \rangle - \langle X_t , \log X_t \rangle \\
& \le \sum_{i=1}^n \lambda_i \Big ( \eta \sum_{i=1}^{t-1} G_i \Big ) \sigma_i (X_t) - \sum \sigma_i \log \sigma_i
\end{align} 
where the first inequality is from Von-Neumann's trace inequality. Since the above inequality is exact when $X_t$ and 
$\sum_{i=1}^{t-1}  G_i$ have the same eigenvector, this conclude the proof of the lemma. 

\end{proof} 

From previous proof, we conclude that the eigenvalue  corresponding to the largest eigenvector  of $X_t$ and $\sum_{i=1}^{t-1}  G_i$ coincide. 


\begin{lemma} 
$X_t $ has  $r \le k $ e. v. of magnitude $1/k$ and has the following form 
\[
X_t = \sum_{i=1}^r \frac 1 k v_i v_i^T + (1-r/k) \frac { P_v^\perp \exp ( \eta \sum_{i=1}^{t-1}  G_i) P_v^\perp } { \Tr (\eta \sum_{i=1}^{t-1} G_i) }, \quad v = [ v_1, \ldots v_r] .
\]
\end{lemma} 

\begin{proof} 
 Let $\sigma_1, \ldots \sigma_n$ be the eigenvalues  of $X_t$ (eigenvector same as  $\sum_{i=1}^{t-1}  G_i$). 
 
 Now let $r=   | \{ i: \sigma_i \ge 1/k \} |$. We know that $ r \le k $ as $\sum_{i=1}^n  \sigma_i = 1, \sigma_i \ge 0$.
 Then 
 \begin{align} 
\sigma_{r+1}, \ldots \sigma_n=  \argmax_{\sum_{i=r+1}^n \sigma_i  = 1 - r/k} \sum_{i=r+1}^n \sigma_i \lambda_i \Big ( \eta \sum_{j=1}^{t-1} G_j \Big ) - \sum_{i=r+1}^n \sigma_i \log \sigma_i
\end{align} 
(Upper bound doesn't matter from dual consideration.) This implies 
  \begin{align} 
 \forall i > r,  \quad  \sigma_i =  \frac { \exp \big (\lambda_i \big ( \eta \sum_{s=1}^{t-1} G_s \big ) \big )} { \sum_j \lambda_j  \exp \big ( \eta \sum_{s=1}^{t-1} G_s\big ) \big )}.
\end{align} 
 
\end{proof} 

Algorithm: Compute $X_t$. 
  \begin{align} 
M_t  = & \exp \big ( \eta \sum_{s=1}^{t-1} G_s \big ), \quad (\lambda_i, v_i), i=1 \ldots k, \; \text{ the top  $k$ eigenvalues and eigenvectors of }  M_t.\\
r^*:= & \argmin_{r \ge 0} \lambda_1 \Big ( \frac { M_t - \sum_{i=1}^r \lambda_i v_i v_i^T (1- r /k)}  { \Tr \big ( \sum_{i=1}^r \lambda_i v_i v_i^T (1- r /k)} \big ) \Big )
\le 1 /k \\
X_t & \leftarrow  \sum_{i=1}^{r^\ast}   v_i v_i^T +  \frac { P_v^\perp M_t P_v^\perp } { \Tr (P_v^\perp M_t P_v^\perp ) } \big (1- r^\ast  /k \big )
\end{align} 



\newpage 
Consider the following optimization: 
\[\tag{*} 
\min_{0 \le \sigma_i \le 1/k, \sum \sigma_i = 1}  \sum \sigma_i \log \sigma_i + C^T \sigma
\]
Observe that if $\sigma^\ast$ is  opt, $\sigma^\ast$ satisfies  if $c_i \le c_j \Longrightarrow \sigma_i \ge \sigma_j$. Monotonicity. 
Algorithm picks 
\[
r= \min_{\ell \ge 0} \Big [ \frac { e^{- c_{\ell+1} } } { \sum_{m > \ell} e^{- c_{m} } } \big ( 1 - \frac \ell k \big ) \le 1/ k \Big ] 
\]
If $\sigma^\ast$ is  opt, let $r^\ast$ be the number of $\sigma_i = 1/k$. From strong duality ( Slater's   condition ), we get for all $i > r^\ast$ (using complimentary 
slackness) 
\[
\log \sigma_i^\ast + 1 + c_i + \beta =0 \Longrightarrow \sigma_i^\ast = e^{- \beta - 1} e^{-c_i}
\]
by dual variable corresponding  to $\sum \sigma_i = 1$. 
Thus we have for all $i > r^\ast $, 
\[
 \sigma_i^\ast = \frac { e^{- c_{i} } } { \sum_{i > r^\ast} e^{- c_{i} } } \big (1- r^\ast  /k \big )
\]
This implies $ r \le r^\ast$. To prove  $ r = r^\ast$, asume  $ r <  r^\ast$, this is a contradiction as this results in lower objective value
 as (*)  is decompossable. 

\newpage 
 \newcommand{\e}{\varepsilon} 
 
  \begin{align} 
\min  \big ( \Tr Y \big )
\end{align} 
subject to the constraints $Y \cdot A_i \ge 1, \| Y \| \le \Tr Y /k, Y \succeq 0$. 

Dual 
 \begin{align} 
\max  \sum_{i=1}^m  x_i 
\end{align} 
subject to the constraints $ \| \sum_{i=1}^m  x_i A_i \|_k \le k, x_i \ge 0$. 

Solve $\varepsilon$-decision  problem.  algorithm 
\begin{align} 
& k = \frac { (1 + \log n ) } \e, \quad \alpha = \frac { \e'} { (1+ 5 \e)k K + 2 (\e')^2 R k} , \quad R = \frac { 256 k K \log n} { \e' \e}, \quad \e'= \frac { \e^2} { 512 k \log n } \\
& \qquad  t \leftarrow 0, \quad x_i^{(0)} \leftarrow \Tr (A_i)/n \\
&\text{while } \| x_i^{(t)}\|_1\le k \text { and } t \le T \\
&\qquad  t \leftarrow t+1 \\
&\qquad P^{(t)} \leftarrow P_s(\sum_{i=1}^m  x_i^{(t-1)} A_i )  \\
&\qquad  \beta^{(t)} \leftarrow \{ i: \langle A_i,  P^{(i)} \rangle \le 1 + \e \}  \\
&\qquad  x^{(t)} \leftarrow x^{(t+1)}+ \alpha x_\beta^{(t-1)} \\
&\text{end }  \\
&\qquad  \text{if }  \| x^{(t)}_i  \| \ge k  \\
&\text{return }  \hat x = \frac 1 { (1+ 10 \e ) k } x^{(t)}  \text{ as dual solution}   \\
&\text{return }  \bar y  = \frac 1 t \sum_{\tau = 1}^t \rho{(\tau)}  \text{ as  primal  solution}   \\
&\text{end }  
\end{align} 

\newpage 
gain matrices $M^{(t)} = \frac \alpha {\e'} \sum_{ i \in B} x_i^{(t-1)} A_i  $
\[
\Psi^{(t)} = \sum_{i=1}^m   x_i^{(t)} A_i  
\]
\[
\delta_i^{t)} = \alpha x_{\beta^{(t)}}^{t-1}   \Longrightarrow x^{(t)} = x^{(0)} + \sum_{r=1}^t \delta^{(r)}
\]

Claim 1: $ \| \Psi^{(0)}  \|_k \le 1$. 


{\bf  Claim 2:}
\[
 \exists  t =0, \ldots T, \quad \langle M^{(0)},  P^{(t)} \rangle \le \frac { 1 + \e} { \e'} \| \delta^{(t)}  \|_1
 \]
 Proof: 
 \[
\langle M^{(0)},  P^{(t)}\rangle = \Big \langle \frac 1 { \e'} \big ( \sum_i \delta_i^{t)}  A_i \big ),   P \Big \rangle \le  \frac { 1 + \e} { \e'} \sum_i \delta_i^{t)} 
 \le     \frac { 1 + \e} { \e'} \| \delta^{(t)}  \|
 \]

{\bf  Claim 3:}
\[
\text{ For }   t =0, \ldots T, \quad  \|x^{(t)} \|_1 \le   (1 + \e) k 
 \]
It follows from $\alpha \le \e' \le \e$. 


\begin{lemma}[spectrum bound] 
$\text{ For }    t =0, \ldots T$, we have 
\[
 \| \Psi^{(t)}  \|_k \le ( 1 + 5 \e) k K + 2 (\e')^2 R k \le ( 1 + 10 \e) k K
\]
\end{lemma} 

\begin{proof} 
We have 
\[
 \| M^{(r)}  \| \le \frac \alpha { \e'}  \| \sum_{i=1}^m x_i^{(t-1)} A_i   \| \le   \frac \alpha { \e'}  \| \Psi^{(t)}  \|_k \le 1. 
\]
From regret bound, 
\begin{align} 
 \e' \frac {   \| \sum  M^{(r)}  \|_k}  k  & \le  \e'  \sum_{r=1}^{t-1}   M^{(r)} \cdot P^{(r)}
 + 2 (\e')^2 R + \log n \\
 & \le (1+ \e)  \| x^{(r)}  \|_1+ \log n + 2 (\e')^2 R \\
 & \le (1+ \e)^2  K+ \log n + 2 (\e')^2 R 
 \end{align} 
 \begin{align} 
  \| \Psi^{(t)}  \|_k \le  \| \Psi^{(0)}  \|_k+ \e'  \| \sum  M^{(r)}  \|_k & \le 1 + (1+ \e)^2  K k + k \log n + 2 (\e')^2 R k \\
 & \le (1+ 5\e)k   K + 2 (\e')^2 R k
 \end{align}

\end{proof} 

\newpage 



\begin{lemma}[Dual exit] 
If $ \| x^{(T)} \|_1 \le R$ then $A_i \cdot \bar Y \ge 1$. 
\end{lemma} 

\begin{proof} 
 Suppose $A_i \cdot \bar Y <  1, \bar Y = \frac 1 T \sum_{r=1}^{t-1} P^{(r)}$. 
\[
U = \{ i: P^{(r)} \cdot A_i \le 1 + \e \} .
\]
by Markov, $|U | \ge \frac \e { 1 + \e} T$. Since $T = R$, 
\begin{align} 
x_i^{(T)} \ge \exp \Big ( \frac \alpha 2 \cdot \frac { \e R} { 1 + \e} \Big ) \ge  \exp \Big ( \frac { \e'} { 4K k} \cdot \frac \e 2   \cdot \frac { 256 \log n k K } { \e \e'} \Big ) 
\ge \Omega(n^4) .
 \end{align} 
 
\end{proof} 

Final result: In $O \Big ( \frac {(\log n)^2 k^2} { \e^4} \Big ) $ iterations, alg terminates. 

Proof:  If Dual exit then the solution is Dual feasible. If primal exit then the solution is primal feasible.

\end{comment}


==> content/techniques.tex <==
\section{Our Techniques}
\label{sec:techniques}

We start by outlining the broad steps underlying the design of our algorithm. To build intuition, we illustrate these ideas in the specific setting where the our data is generated according to a mixture of $k = 1/\alpha$ well separated distributions with bounded covariance; i.e $X_i \thicksim k^{-1} \sum_{i = 1}^k \mc{D}_i$ with $\mu(\mc{D}_i) = \mu_i$. One possible approach that is inline with current approaches to clustering mixtures of distributions is to first identify a single cluster center, $\mu_1$ for example, identify and remove the data points corresponding to $\mc{D}_i$ and iterate the procedure until we have recovered all the cluster centers. We now describe an inefficient algorithm, operating according to the paradigm described previously, which provably returns good approximations to the cluster centers. 

\paragraph{Inefficient Algorithm:} Our inefficient algorithm attempts to identify a set of data points which have bounded covariance. It then proceeds to label this set of points as belonging to the first cluster and then iterates this procedure on the data points left after the removal of these points. Instead of making hard assignments of data points to clusters, we allow the algorithm to make fractional assignments. This corresponds to a to solving the following optimization problem (Note that the weights for each data point are bounded by $\frac{1}{\alpha N}$ as each point in a cluster constitutes a $\frac{1}{\alpha N}$ part of the cluster):

\begin{align*}
    \min_{\substack{0\le w_i\le \frac{1}{\alpha N} \\ \sum_{x\in X} w_i = 1 \\ \forall x \in X}}  \norm{\sum_{x\in X} w_i (x - \hu(w)) (x - \hu(w))^{\transp}}.
\end{align*}

Having solved the above optimization problem to obtain a minimizer, $\bar{w}$, the algorithm then adds $\mu(\bar{w})$ to the list of discovered clustered centers and repeats the procedure by ``removing'' the data points assigned to this cluster. Note that since we assign soft weights to the data points, ``removing'' a data point corresponds simply to decreasing the amount of mass that may be assigned to a data point in subsequent iterations of the algorithm. For example, in the second iteration, we enforce the constraint that $w_i \leq \frac{1}{\alpha N} - \bar{w}_i$. Therefore, in general the algorithm maintains a list of weight budgets, $\{b_i\}_{i = 1}^N$, for each data point specifying the possible weight values for that point in subsequent steps. By iterating this procedure $k$ times, we eventually recover $k$ cluster centers and the algorithm terminates. This is because the total amount weight assigned to all data points is $k$ and we remove $1$ amount of weight in each step. A slight technicality is that a $.01$ fraction of weights removed in a particular step do not belong to the cluster extracted in the step. To accommodate  for this we will initialize $b := \frac{1}{0.99\alpha N}$, the initial budget of weights for each data point and iterate the algorithm for $\frac{1}{0.99\alpha}$ iterations. Our algorithm outputs a list of size $\approx 1.01 k$ but this is not an issue for our list-decodable setting. We now present a brief proof outline establishing the correctness of the aforementioned procedure:

\begin{proof}[Proof Outline]
The proof is by contradiction. Fix a cluster center, $\mu$, and let $I$ denote the set of points belonging to the particular cluster. Assume that every iteration failed to produce a $\hat\mu$ satisfying $\norm{\hat\mu - \mu} \leq \frac{20}{\sqrt \alpha}$. Then, in the first iteration we know $\sum_{x \in I}\bar w \leq \frac{1.01\alpha}{400}$ through a standard application of the second moment bound as in the first iteration, the covariance matrix corresponding to $\bar{w}$ must have smaller spectral norm than the covariance matrix corresponding to any individual cluster. By carefully keeping track if the amount of mass removed from points in $I$, one can establish similar guarantees for every iteration of the algorithm. Therefore, in every iteration, the amount of mass removed from $I$ is less than $\frac{\alpha}{200}$. Since the sum of the inlier weight is initialized to be $\sum_{x \in I}b_x = \frac{1}{0.99}$, we have at the conclusion of the second to last iteration a dataset with satisfying $\sum_{i \in I} b_i = 1$.  This ``set'' of points which only belong to $I$, will then be removed in the last iteration and will result in an estimate $\hat{\mu}(\bar{w})$ close to $\mu$ establishing the contradiction.
\end{proof}

However, the main drawback with the approach outlined previously is that it is not clear how to quickly obtain a good solution to the optimization problem considered in the previous step. We now introduce some notation to declutter subsequent exposition:

\begin{equation*}
    f_b(\nu) = \min_{0 \leq w_i \leq b_i} \max_{\substack{M \succcurlyeq 0\\ \Tr (M) = 1}} \inp{\sum_{i = 1}^N w_i (X_i - \mu)(X_i - \mu)^\top}{M} = \min_{0 \leq w_i \leq b_i} \norm*{\sum_{i = 1}^N w_i (X_i - \mu)(X_i - \mu)^\top}.
\end{equation*}

Note that the min and the max in the previous formulation can be exchanged by von Neumann's Min-max theorem and consequently, an optimal solution $(M^*, w^*)$ exists for the above program. Therefore the previous algorithm can be seen as attempting to find $\nu$ to minimize $f_b$ in each iteration. One approach is doing so is to start with an estimate $\nu$ and iteratively improve the estimate till the value of $f_b$ is small. This is the approach taken in \cite{CDG}, where it was deployed for robust estimation problems under the $\eps$-contamination model for $\eps < 1/2$. In this setting, the learner is given access to $N$ data samples, $\{X_i\}_{i = 1}^n$ generated in the following way:

\begin{enumerate}
    \item First, $\{Y_i\}_{i = 1}^N$ are generated IID from a distribution, $\mc{D}$, with covariance bounded by $\sigma^2 I$.
    \item An adversary then inspects the samples and corrupts an arbitrary $\eps$ fraction of them.
\end{enumerate}

The goal of the learner is then to estimate the mean of $\mc{D}$, denoted by $\mu(\mc{D})$, up to the information-theoretically optimal error of $O(\sqrt{\eps} \sigma)$. For the $\eps$-contamination setting, $b_i = \frac{1}{(1 - O(\eps))N}$ for all $i$. It can be shown that any candidate, $\nu$, for which $f_b(\nu)$ is small is close to the true mean $\mu(\mc{D})$. Therefore, given a particular, $\nu$, one can efficiently check if $\nu$ is close to $\mu(\mc{D})$ by computing the value of the program. The key idea behind \cite{CDG} is that given a candidate estimate, $\nu$, the value of the above program serves a proxy for the distance to the true mean. And furthermore, when $\nu$ is far from the mean, the solution, $M^*$, is well aligned with the vector $(\mu(\mc{D}) - \nu)$. In particular, its top singular vector can then be used to perform a gradient descent step guaranteed to move closer to $\mu(\mc{D})$. By iterating the above procedure, one converges linearly to a good estimate of $\mu{\mc{D}}$.

However, this approach runs into difficulties in the setting of list-decodable learning where one instead sets $b_i = \frac{1}{\alpha N}$ as the number of inlier data points is $\alpha N$. The cost function, $f(\nu)$, no longer serves as a proxy for the distance to $\mu(\mc{D})$. To see this, consider the simple special case of the list-decodable learning setting where the data is distributed according to a mixture of $(1 / \alpha)$ distributions with bounded covariance. Without any knowledge of which mixture component represents the true inliers, the result of $f_b(\nu)$ can be an arbitrarily bad estimate of $\norm{\nu - \mu(D)}$. Without a clear interpretation of $f(\nu)$ in terms of the distance to $\mu(\mc{D})$ for example, it is unclear how to argue about the effect of an update with the top singular vector of $M^*$.

To illustrate the above difficulties, consider the simpler setting of a mixture of $k = 1 / \alpha$ distributions with bounded covariance, $X \thicksim k^{-1} \sum_{i = 1}^k \mc{D}_i$. Even in this simple setting, $f_b(\nu)$, only approximates the distance to the closest cluster up to a factor of $1 / k$. To see this, consider a mixture where the mixture components have means at $\pm \lambda e_{i}$ for large $\lambda$ and suppose the test point is $\nu = 0$. We have $f_b(0) \approx \frac{\lambda^2}{k}$. This can be accomplished by setting $w_x = 1 / N$ for all $x \in X$ furthermore, $M^* = d^{-1} \bm{1} \bm{1}^\top$ achieves this value. Therefore, even in this simple setting, $f_b$ only approximates the distance to the closest cluster up to a factor of $1 / k$ and furthermore, the top singular direction of $M^*$ has only a $1 / \sqrt{k}$ overlap with the direction to the closest cluster. Therefore, to guarantee progress to the closest cluster, one needs to run at least $k \log k$ steps of gradient descent. Additionally, it is unclear which orientation of the top singular vector of $M^*$ is the ``true'' descent direction. Trying both possibilities for the first $k$-steps descent results in us computing $f_b$, $O(k^k)$, times. This runtime is intractable even for mildly super constant values of $k$; for example, $k = \log d$.\ynote{Contract or remove this paragraph.}

\subsection{Our Approach}
\label{ssec:ourapproach}

To aid in exposition, we again restrict ourselves to the simpler problem where the data is distributed according to a mixture of $k = (1 / \alpha)$ distributions with bounded covariance; that is $X_i \thicksim \sum_{i = 1}^k k^{-1} \mc{D}_i$ and let $T_i$ denote the set of points in each cluster $i$. Before we proceed to describe our approach, we first introduce the nation of a Fantope which is a subset of the set of positive semidefinite matrices parameterized by a single positive integer, $l$:

\begin{equation*}
    \mathcal{F}_l = \{M: \norm{M} = 1 \text{ and } \Tr (M) = k\}.
\end{equation*}

We now introduce the following generalization of the min-max problem considered in the previous section:

\begin{equation*}
    f_b^l(\nu) = \min_{0 \leq w_i \leq b_i} \max_{M \in \mathcal{F}_l} \inp{\sum_{i = 1}^N w_i (X_i - \mu)(X_i - \mu)^\top}{M} = \min_{0 \leq w_i \leq b_i} \norm*{\sum_{i = 1}^N w_i (X_i - \mu)(X_i - \mu)^\top}_l \leq C \sigma^2
\end{equation*}

where $\norm{A}_l$ denotes the sum of the top-$l$ singular vectors of $A$. Note that when $l = 1$, $f^l_b$ corresponds to the function, $f_b$. For our current setup of second moment bounded mixtures, we pick $l = k$ in the above formulation. As before, consider a candidate estimate $\nu$ that is farther than $O(\sqrt{k})$ away from the means of each of the $\mc{D}_i$. In this setting, one may choose $M \in \mc{F}_l$ to be the projection matrix onto the subspace containing the means of each of the $\mc{D}_i$. With this particular choice, we see that the value of $f^k_b(\nu)$ is indeed a good approximation to the distance to the closest cluster; it can never by significantly larger by simply choosing the $w_i = k / N$ for the points belonging to the closest cluster. Furthermore, one can establish that the mean of the closest cluster relative to the current estimate $\nu$ is almost completely contained in the top-$O(k)$ singular subspace of $M^*$. We may now project all the data points onto this subspace. The second observation is that a random data point on the closest cluster is $O(\sqrt{k})$ away from the projection of the mean of the cluster. Since this subspace almost completely contains the mean of the closest cluster, a random projected data point from the cluster is also significantly closer to the true mean. By picking $\tilde{O}(k)$ random data points, one can ensure picking a point significantly closer to the mean. We can efficiently check if we have made progress by computing the value of $f_b^l$ at the new estimate. By iterating this procedure we converge to within $O(\sqrt{k})$ of the mean of a cluster center.

However, this approach still has two main drawbacks:

\begin{enumerate}
    \item How does one iterate this procedure once one finds one cluster center?
    \item How can the above intuition be extended to the general list-decodable setting?
\end{enumerate}

Let us assume without loss of generality that we have converged close to the first cluster consisting of the points $T_1$. In an ideal setting, one would like to simply remove the data points corresponding to the discovered cluster and iterate the procedure. One would hope that the weights, $w^*$, are entirely concentrated on the points from the discovered cluster. However, this is not quite true as $w^*$ can still have significant mass on points from other clusters. Nevertheless, we are able to establish the following guarantee on $w^*$. Let $X_1 \dots X_N$ be an ordering of the data points such that $\Pi_V (X_1 - \nu) \leq \Pi_V (X_2 - \nu) \dots \leq \Pi_V (X_N - \nu)$ where $V$ is the top-$k$ singular subspace of $\sum_{i \in [N]} w_i (X_i - \nu)(X_i - \nu)^\top$ and let $t^* = \max\{t: \sum_{j = 1}^t w_j \leq 0.5\}$. Then $\sum_{j \in T_i \cap [t^*]} w_i \leq 1 / (10^3 k)$. Therefore, one may remove safely remove the points in $[t^*]$ without destroying too much of the other clusters. In reality, we show a ``soft'' version of the previous statement where we do not completely remove points but rather downweight them in subsequent iterations but the intuition still applies. By iterating this procedure, we may progressively eliminate clusters from the dataset and eventually recover all the cluster centers; since we remove at least $\alpha N / 2$ points in each iteration, we only iterate this procedure at most $O(1 / \alpha)$ times. 

In the general list-decodable learning set-up, our data is not quite as structured and we instead establish the following win-win scenario -- either we converge close to the mean of $\mc{I}$ or the set $[t^*]$ satisfies $\sum_{j \in \mc{I}} w_i \leq 10^{-3} \alpha$. Note that due to the lack of structure in the data distribution, such guarantees cannot be obtained for the other ``clusters'' in the data. Nevertheless, the previous results show that by iteratively repeating the procedure, one either obtains a good estimate of $\mu(\mc{I})$ or one eliminates a substantial fraction of outliers. Thus within $O(1 / \alpha)$ steps, the algorithm terminates and one of the recovered estimates is close to desired mean. Next, we tackle the question of how to compute $f^k_b$ efficiently.

\subsection{Generalized Packing/Covering Solvers and Improved Power Method Analysis}
\label{ssec:genpacktech}

We start by considering the simpler problem of computing $f^1_b(\nu)$. The approach taken in \cite{CDG} is to reduce the problem to a packing sdp via the introduction of an additional parameter $\lambda$; specifically, they solve the following packing sdp:

\begin{equation*}
    \label{eqn:packptz}
    \begin{gathered}
    \max_{w_i \geq 0} \sum_{i = 1}^N w_i \\
    \text{s.t } \norm{\sum_{i = 1}^N w_i (X_i - \nu)(X_i - \nu)^\top} \leq \lambda \tag{Packing-SDP}\\
    w_i \leq b_i
\end{gathered}
\end{equation*}

for which there exist fast linear-time solvers \cite{peng2012faster,ALO16}. It can be shown that the value of the above program when viewed as a function of $\lambda$ is monotonic, continuous and attains the value $1$ precisely when $\lambda = f_b(\nu)$. Therefore, by performing a binary search over $\lambda$, one obtains accurate estimates of $w^*$ and $f_b(\nu)$. 

However, a similar approach for the problem of compute, $f^l_b (\nu)$ results in the following SDP:

\begin{gather*}
    \max_{w_i \geq 0} \sum_{i = 1}^N w_i \\
    \text{s.t } \norm{\sum_{i = 1}^N w_i (X_i - \nu)(X_i - \nu)^\top}_l \leq \lambda \\
    w_i \leq b_i
\end{gather*}

which does not fall into the standard class of packing sdps. We extend and generalize fast linear time solvers for packing/covering sdps from \cite{peng2012faster} to this broader class of problems. However, this generalization is not straightforward. 

To demonstrate the main difficulties, we will delve more deeply into the solver from \cite{peng2012faster}. We assume without loss of generality that $\nu = 0$ and state the packing/covering primal dual pairs they consider:

\begin{table}[h]
\centering
\begin{tabularx}{\textwidth}{ >{\centering\arraybackslash}X | >{\centering\arraybackslash}X }
  Covering (Primal) & Packing   (Dual) \\
  \begin{gather*}
      \min_{M} \Tr{M} \\
      \text{Subject to: } \inp{A_i}{M} \geq 1\\
      M \succcurlyeq 0
  \end{gather*} & 
  \begin{gather*}
      \max_{w_i \geq 0} \sum_{i = 1}^N w_i \\
      \text{Subject to: } \sum_{i = 1}^N w_i A_i \preccurlyeq I
  \end{gather*}
\end{tabularx}
\end{table}

The solver of \cite{peng2012faster} start by initializing a set of weights, $w_i$, feasible for \ref{eqn:packptz}. Subsequently, in each iteration, $t$, they first compute the matrix 

\begin{equation*}
 P^{(t)} = \frac{\exp (\sum_{i = 1}^N w_i A_i^\top)}{\Tr{\exp (\sum_{i = 1}^N w_i A_i^\top)}}.
\end{equation*}

The algorithm then proceeds to increment the weights of all $i$ such that $\inp{P^{(t)}}{P^{(t)}} \leq (1 + \eps)$ for a user defined accuracy parameter, $\eps$, by a multiplicative factor. Intuitively, these indices correspond to ``directions'', $A_i$, along which $\sum_{i = 1}^N w_i A_i^\top$ is small and therefore, their weights can be increased in the dual formulation. By incorporating a standard regret analysis from \cite{DBLP:journals/jacm/AroraK16} for the matrices, $P^{(t)}$, they show that one either outputs a primal feasible, $M$, with $\Tr M \leq 1$ or a dual feasible $w$ with $\sum_{i = 1}^N w_i \leq (1 - \eps)$.

The construction of our solver follows the same broad outline as in \cite{peng2012faster}. While the regret guarantees we employ are a generalization of those used in \cite{peng2012faster}, they still follow straightforwardly from standard regret bounds for mirror descent based algorithms \cite{DBLP:journals/corr/abs-1909-05207}. Instead, the main challenge of our solver is computational. The matrix $P^{(t)}$ can be viewed as a maximizer to $f(X) = \inp{X}{F} - \inp{X}{\log X}$ where $F = \sum_{i = 1}^N w_i A_i$ in $\mc{F}_1$. In our setting, we instead are required to compute the maximizer of $f$ in $\mc{F}_l$ which we show is given by the following: Let $H$ and $\tau^*$ be defined as:

\begin{equation*}
    H = \exp(F) = \sum_{i = 1}^m \lambda_i u_i u_i^\top \text{ with } \lambda_1 \geq \lambda_2 \ldots \geq \lambda_m > 0 \text{ and } \tau^* = \max_{\tau > 0} \lbrb{\frac{\tau^*}{\sum_{i = 1}^m \min (\tau, \lambda_i)} = \frac{1}{l}}.
\end{equation*}
 
Then, we have:
\begin{equation*}
    P^{(t)}_l = \min_{X \in \mc{F}_l} f(X) = \frac{l}{\Tr \sum_{i = 1}^m \min(\lambda_i, \tau^*) u_iu_i^\top}\cdot \sum_{i = 1}^m \min(\lambda_i, \tau^*) u_iu_i^\top.
\end{equation*}

While the matrix, $P^{(t)}$, can be efficiently estimated by Taylor series expansion of the exponential function (See \cite{DBLP:journals/jacm/AroraK16}), we need to estimate $P^{(t)}_l$ which is given by a careful truncation operation on $\exp (F)$. Note that given access to the exact top-$l$ eigenvectors and eigenvalues of $\exp(F)$, one can efficiently obtain a good estimate of $P^{(t)}_l$. However, the main technical challenge is establishing such good estimates given access only to \emph{approximate} eigenvectors and eigenvalues of a truncated taylor series approximation of $H$. 

One of the main insights of our approach is that instead of analyzing the truncation operator directly, we instead view the matrix. $P^{(t)}_l$ as being the maximizer of $g(X, F) = \inp{F}{X} - \inp{X}{\log X}$ with respect to $X$. We then subsequently show that maximizer of $g(X, \wt{F})$ is close to $P^{(t)}_l$ for some $\wt{F}$ close to $F$ makes crucial use of the fact that $\log X$ function is operator monotone. Our second main piece of insight is that if our approximate eigenvectors and eigenvalues, denoted by $(\wh{\lambda_i}, i_i)_{i = 1}^l$ satisfy:

\begin{equation*}
    (1 - \eps) \sum_{i = 1}^l \wh{\lambda_i} v_i v_i^\top + \mc{P}_V^\perp H \mc{P}_V^\perp \preccurlyeq H \preccurlyeq (1 + \eps) \sum_{i = 1}^l \wh{\lambda_i} v_i v_i^\top + \mc{P}_V^\perp H \mc{P}_V^\perp,
\end{equation*}

where $V$ is the subspace spanned by the $v_i$ and $\mc{P}^\perp_V$ is the projection onto the orthogonal subspace of $V$, then our approximate truncation operator can be viewed of as the \emph{exact} maximizer of $g(X, \wt{F})$ for some $\wt{F}$ close to $F$. From the previous discussion, this means that our truncation operator operating on the approximate eigenvectors $v_i$ is a good estimate of $P^{(t)}_l$. However, standard analysis of methods for the computation of eigenvalues and eigenvectors do not yield such strong guarantees \cite{DBLP:conf/nips/ZhuL16,DBLP:conf/nips/MuscoM15} \ynote{put more reference here}. The final contribution of our work is a refined analysis of the power method that yields the required stronger guarantees \footnote{While our guarantees scale with $1 / \eps$ as opposed to $1 / \sqrt{\eps}$ as in \cite{DBLP:conf/nips/MuscoM15}, we suspect this dependence may be improved using techniques from \cite{DBLP:conf/nips/MuscoM15}.}.

==> content/todo.tex <==
\section{TODO}

Overall paper tasks:

\begin{enumerate}
    \item Write and refine introduction (Do carefully tomorrow)
    \item Check technical consistency and correctness (Would ideally like to finish this today)
    \begin{enumerate}
        \item Unify notation across different parts of the paper
        \item Make a pass to ensure correctness of technical portions of the paper
    \end{enumerate}
\end{enumerate}
